Let the Cloud Watch Over Your IoT File Systems

Smart devices produce security-sensitive data and keep them in on-device storage for persistence. The current storage stack on smart devices, however, offers weak security guarantees: not only because the stack depends on a vulnerable commodity OS, but also because smart device deployment is known weak on security measures. To safeguard such data on smart devices, we present a novel storage stack architecture that i) protects file data in a trusted execution environment (TEE); ii) outsources file system logic and metadata out of TEE; iii) running a metadata-only file system replica in the cloud for continuously verifying the on-device file system behaviors. To realize the architecture, we build Overwatch, aTrustZone-based storage stack. Overwatch addresses unique challenges including discerning metadata at fine grains, hiding network delays, and coping with cloud disconnection. On a suite of three real-world applications, Overwatch shows moderate security overheads.

==> assumptions.tex <==
% !TEX root = main.tex
\subsection{Assumptions}

execution characteristics, fs behaviors, etc.

==> benchmark.tex <==
% !TeX root = main.tex

\subsection{Kernel microbenchmarks}


==> benchmarks.tex <==
% !TEX root = main.tex

\subsection{Microbenchmarks}

\Paragraph{Benefit of energy efficiency}

==> design-choice.tex <==
\subsection{Design space exploration}
\note{then given previous arguments, this section mainly explore design space under two assumptions 1) cloud-local pair is needed, 2) replicated execution is needed}
\begin{comment}
\xzl{Structure this section as a set of key ideas}

\xzl{addressing the following questions}

\note{Rewrite the flow: it's ok to highlight key ideas in bulletpoints, but the ideas should flow naturally and logically. Better not write like ``I notice the vulnerability here so I fix there'' kind of style.}

\begin{enumerate}
\item 
what fs modifications are required? 
\item 
which components go to which world?
\item 
how do two worlds interact?
\item 
what's the role of the cloud? the secure world (e.g. tracking block type)? the normal world? 
\item 
what's the interface of the secure page cache?
\item 
what blocks are exposed to the normal world? 
\item 
how do open(), read(), and write() work?
\item 
how do unlink(), chdir(), and rmdir() work?
\end{enumerate}

\end{comment}

%Motivated by the challenges and rationales above, 

In this section, we explore the design space for cloud-backed file systems and then present our choice.
% introduce our key idea that we run a file system replica with only metadata on the trusted cloud backend for security.

%By far, we have discussed why even with the hardware-based mechanism, file system security, especially verifiable persistence, still can not be ensured solely on the local side and how the cloud can help complete the puzzle.



%\subsection{Goals and Challenge}

%\note{move goals to sec 2}

%\paragraph{Design goals} 
%Given the status quo of IoT devices, it seems not feasible to address these three challenges altogether.
\begin{comment}
\paragraph{Non-repudiable I/O} 
It's not enough by simply securing the cached read/write.
Without being securely backed by underlying block devices, a malicious file system can easily twist the application's will, for example, by simply dropping the write requests or passing a wrong block number to the block layer.
In our design, we propose the secure world handle I/O requests passed from normal world, which is a block number and a reference to a memory page.
Note that since this memory page belongs to the application, it is hosted by the secure cache.
Therefore, in handling these requests, we naturally gurantee the data integrity as well as confidentiality.
Then, the secure world performs I/O and thus ensures the execution integrity of these requests, i.e. the content is written honestly to its assigned block.
We then discuss how we guanrantee the correctness of these requests in section \ref{sec:cloud}.
\end{comment}

%In achieving these three design goals, we face the following unique challeges 1) file system, even the OS is untrusted, which allows for a giant attack surface 2) the performance constraint is tight, which doesn't allow for a hypervisor.
%1) the intrinsic complexity of file system prevents itself from being included in TCB, 2) the UNIX common file model prevents a more ``precise'' protection\note{rephrase} and 3) the file system does not understand the security semantics. 





%Until verified, otherwise the application continue.


%We trust the secure boot of TrustZone and the TEE provided by it. We also trust the world switch between secure world and normal world is secure (i.e. cannot be hijacked). In addition, we trust the cloud verification server. The communication between IoT device and the cloud is encrypted\note{discuss man-in-the-middle attack?} and that the verification message cannot be forged. Note that we are aware of side channel attack\note{cite} such as bus spoofing\note{cite}. However, the physical attack is not in our scope. 

%\subsection{IoT security is not a one-man job}

%To this end, we propose to extract secure primitive from commodity file system into secure plane, aided by a lightweight cloud verfication server. %The design is as follows. 


%In a nutshell, for each file operation, TEE sends it to local untrusted fs and also the cloud trusted replica.
%If the operations are verified, local fs let them through; otherwise, they'll get rejected and then XXX.
%The design is discussed in detail below.



\begin{comment}
\paragraph{Integrity invariants}
To keep the interfaces as narrow as possible, we identify three invariants to meet for a secure file system operation on a local device as shown below. 
\begin{enumerate}
\item The blocks to be written are intact along the path.
\item The content to be written to the blocks are intact.
\item The communication with underlying block device is intact.
\end{enumerate}

\note{more high-level description, naive though}
\begin{enumerate}
\item The path from block to memory is intact.
\item The path from memory to block intact.
\end{enumerate}
\end{comment}

%\subsection{Design Space Exploration}
\label{sec:exploration}

%\yiying{If you only have one subsection, you don't need a subsection and can just put everything under the section.}

%\paragraph{A space of cloud-backed file systems}
\paragraph{What \textit{least} knowledge does cloud need?}
%\note{even move related work here? keywords include: remote attestation, operation shipping, provable data possession, principle of equivalence(used to checkpoint)}
In designing such a distributed file system whose major goal is to provide aforementioned strong security guarantees, we keep the question in mind: \textit{what least knowledge does cloud need}, because even though the cloud is a must to achieve our security goals, we still want to minimize the potential attack surface.

To answer this question, in Figure~\ref{fig:spectrum} we lay out a broad spectrum of networked systems based on how much knowledge the cloud has (i.e., how data and metadata is replicated).
%The ideas of distributing file system functions and data are not new. 
%Figure \ref{fig:spectrum} shows a broad spectrum of cloud-backed file systems, based on \textit{how the data is replicated} between a local device and a cloud server. 
%On the bottom left sits the systems \cite{cfs} where neither metadata or data is replicated, e.g., local-only file systems or networked file system. In the latter case, the local device's major goal is to cache file contents. 
On the bottom left sits the systems \cite{cfs} where neither metadata nor data is replicated and there is \textit{only} one copy of metadata and data, as exemplified by a networked file system (e.g., Linux NFS). 
%In the latter case, the local device's major goal is to cache file contents. 
On the top left sits distributed file systems~\cite{coda,dropbox}, where the cloud and local side keeps distinct metadata themselves and only data is replicated to the cloud.
The top right includes remote execution systems~\cite{clonecloud,maui} that replicate all the metadata/data on both the local device and the cloud, which also often replicate all file operations on both sides. %\note{this is flip-flop.. MAUI...}

Almost all prior systems replicate user data to the cloud.
In contrast, we argue to avoid so for securing IoT file systems, 
because i) we do not necessarily entrust the cloud for user data confidentiality~(\S\ref{sec:bkgnd:security}),
and ii) the network bandwidth, especially that of uplink, is limited~(\S\ref{sec:backgnd:rationale}).

%The distributed file systems sit at one end of the spectrum, which include  HDFS, Dropbox and Coda\cite{hdfs,dropbox,coda}.
%In such systems, the cloud does most of the work, including (optionally) encrypting and storing the data.
%At the other end sits file systems including CFS and NCryptfs\cite{cfs,ncryptfs}, which provides local encryption service as a mount. %user can choose to store data locally or remotely.
%We also take systems such as MAUI, CloneCloud\cite{maui,clonecloud} into consideration, which offload local tasks to the cloud for remote execution and require a coordination between the local and cloud.
%Since local execution is the majority, we position them closer to the local end in this spectrum.

%The distributed file systems sit at one end of the spectrum, which include  HDFS, Dropbox and Coda\cite{hdfs,dropbox,coda}.
%In such systems, the cloud does most of the work, including (optionally) encrypting and storing the data.
%At the other end sits file systems including CFS and NCryptfs\cite{cfs,ncryptfs}, which provides local encryption service as a mount. %user can choose to store data locally or remotely.
%We also take systems such as MAUI, CloneCloud\cite{maui,clonecloud} into consideration, which offload local tasks to the cloud for remote execution and require a coordination between the local and cloud.
%Since local execution is the majority, we position them closer to the local end in this spectrum.



\begin{figure}[t!]
	\centering
	\includegraphics[width=0.35\textwidth{}]{./figs/design_space} 
	%	\includegraphics[scale=0.35]{./figs/spec} 
	%\missingfigure[figwidth=6cm]{Juno platform power instrumentation}
	\vspace{5pt}		% use as needed
	\caption{The design space for cloud-backed file systems, plotted based on how user data and metadata are distributed.
		%Replicate-none means conceptually the user doens't operate on a local file system entity which replicates metadata and data on disks although she may continue to operate when disconnected as done in Coda. 
		%(\textbf{have to be clear that replicate-none means all metadata+userdata in cloud.}
	}
	\label{fig:spectrum}
	\vspace{-10pt}		% use as needed
\end{figure}

%Therefore, in designing such a system that incorporates the cloud and local, targets low overhead, and most importantly, guarantees the four security properties, we seek to answer the following question: what \textit{the most} should a local file system do and \textit{the least} can the cloud do?

%Given the spectrum, in the following pragraphs, we seek to answer the question: what \textit{the most} should a local file system do and \textit{the least} can the cloud do?

\paragraph{Our design point}
\note{should be tied to security and talk less about performance}
Towards securing IoT file systems, we advocate replicating only the metadata but not the user data to the cloud, as shown in the bottom right part of Figure~\ref{fig:spectrum}. 
As a result, the cloud executes a \textit{metadata-only} file system replica, and is able to validate the legitimacy of any data operations to be performed on the IoT device, defeating \textit{Iago attack} caused by delegating file operations to the commodity file system. 
By avoiding replicating the user data to the cloud, we avoid trusting the cloud for user data confidentiality or integrity as there is no data at all. %and also reduce network traffic. 
%By keeping an untrusted metadata replica on the device, we allow the local file system to operate independently of the cloud, and thus improve performance in case of poor network connectivity.
%Note that by locking the user data solely in the local device, we're able to achieve near-native performance and operational autonomy when disconnected.

%\yiying{this part needs a lot more elaboration}



%2) spotty connectivity, which is not uncommon, prevents the device from becoming fully distributed and will harm real-time on-device analytics, 
%2) before sending the data, encryption is needed if privacy is valued, which lays extra burden on the performance, 
%3) even though encrypted, outsourced data is still in fear of privacy leakage.
%However, entrusting the data and metadata fully to the cloud (e.g. through NFS) as shown in the left end of the figure makes things worse because in addition to the inheritage of all drawbacks of replicate-all approach, it also loses operational autonomy.



\begin{comment}
\paragraph{Local-most is infeasible} \note{a.k.a secure monitor is not a panacea?}
A naive approach will be adopting a local-most system which maximizes the usage of TEE hence achieving the smallest overhead.
With a little faith in file system integrity, it is feasible to achieve data confidentiality, integrity, and freshness.
However, in achieving the fourth goal (i.e. verifiable persistence), the system has to inevitably include the whole file system and block driver into its TEE otherwise there's no way for the system to tell if the block it is writing to is legal or not, as discussed in \S\ref{sec:motiv}.
What's worse, modern file systems are complex, easily with tens of thousands lines of code and rely heavily on kernel services such as memory management, which is not suitable for TEE.
Therefore, It'll be impractical and infeasible to carve out the file system and shove it into TEE.
\end{comment}

\begin{comment}
\paragraph{...Nor is Cloud-most}
Another plain solution is to ``dropbox'' the whole storage, turning the device into a client in a distributed system.
However, we argue this is also infeasible in the IoT scenario for the following reasons:
1) the current bandwidth may not suffice for data transfer of devices not connected to high-speed network, 
2) spotty connectivity, which is not uncommon, prevents the device from becoming fully distributed and will harm real-time on-device analytics, 
3) encryption is needed before sending the data if privacy is valued, which lays extra burden on the performance, 
4) even though encrypted, outsourced data is still in fear of privacy leakage.
\end{comment}

%\paragraph{Implications of the joining of another party}
%\paragraph{In trusting the untrusted cloud}


\begin{comment}
As discussed before, the cloud is trustworthy in terms of availability and reliability thus being used mostly as backup storage or 
Motivated by such an assumption about the cloud, we start from a unique angle: when the cloud is trusted, what can we do to bring security to their clients (i.e. IoT devices)?
Note that it doens't mean we can include arbitrarily many components of the cloud into our TCB for free, instead it means that we can trust the cloud no more, and no less, which has the following implication: what the previous systems are hard to achieve (i.e. verifiable persistence) can now be easily achieved in a system aided by the cloud. 

Prior work (distribtued file sytem) trusts the overall security of the cloud 
Some dont trust the mangement (i.e encrypting the data before uploading)
Some work doenst trust the overall which advocates public auditing
We think the cloud can be trusted no more and no less, meaning the integrity of storage stack can be trusted.
\end{comment}

\begin{comment}
\paragraph{Summary}
In the eternal war of identifying TCB, \textit{what amount of data} should be exposed or kept secure always remains an everlasting yet essential question.

In answering this question, our insight is to only protect data itself by leveraging hardware-enforced TEE and to verify the legitmacy of control path by having the cloud as an overwatch.
It's also worth noting that our design principles are \textit{not} a specification, instead, are only a set of guidelines. 
%another security monitor but a generalized paradigm. 
The security functionality shall be able to map any TEE regardless of its underlying hardware and the implementation includes but is not limited to security monitor; 
the differentiated data shall not limit to directory file block and regular file block. 
It can include superblock, but should be taken cautiously;
the cloud can potentially run a full replica as Secloud \cite{secloud}, but one should keep in mind that its major responsibility is to watch over the local device.
\end{comment}


\begin{comment}
\subsection{Design Choices}
\note{can cut}
By trusting the cloud file system replica, we present a suite of three choices. 

%\note{writing design principle: defining the principle, describe the principle, why this principle, a set of benefits}
%\paragraph{Separating Local File System Functions}
\paragraph{Protect data, not control}
We separate the local file system's data functions from the control functions.
%The data function, guarded by TEE, protects data, and handles a minimal set of secruity-critical operations;
The data function handles actual data move, such as reading data from page cache to a user buffer, and flushing page cache to  a disk block;
the control function executes the control logic of the file system, including maintaining directory structures, managing page caches and blocks, \note{more?}
In modern OSes, the control functions are often complex and fast-evolving, while the data functions are lean and stable.
For instances, the recent Linux kernel has XXX SLoC in XXX and only XXX SLoC in its block layers...

We protect the data functions in the TEE while leaving the control functions in the normal world.
As a result, we shield the data functions from the vulnerable control functions and the underlying OS. 
After separation, our TCB only includes the data functions, the TEE, and the underlying hardware. 


%the control function, sitting in normal world, executes the complex control logic of the original file system.





%in order to leverage TEE as well as minimizing TCB.

%The security responsibilty, guarded by TEE, protects data, and handles a minimal set of secruity-critical operations.
%It issues file system requests (e.g. open, write, close) out to the normal file system;
%it protects security-critical data structures such as page cache, which will be discussed in more detail in section \ref{sec:cache};
%it also runs a secure block driver.
%This ensures our security principles are satisfied. 

%The functionality responsibility, sitting in normal world, preserves the rich functionalities of the original file system.
%It handles requests sent from the TEE and provides services such as file path lookup in locating a file, block allocation in creating a file.
%like any other normal file systems do. 
%It performs most operations .
%However, services provided by the REE file system are NOT trusted.
%In the following paragraphs we'll discuss how we can trustedly utilize these untrusted services.

\paragraph{Cloud as the Overwatch}
%As has been discussed in section \ref{sec:cloud}, to guard the complete file system security we need the cloud to \textit{shepheard} the local file system.
As an essential component, the cloud \textit{watches over} the local file system on by providing feedbacks to the local pending file system operations.
These operations are forwarded to the cloud, and upon receiving, the cloud will replay them on the file system replica that has only the \textit{metadata} and returns the verification results back to local devices.

If the operations on both sides match, which is the case for an untampered device, the verification can succeed, otherwise, the verification will fail.

\paragraph{Differentiating File System Data}
Since we rely on the cloud watch for file system correctness, we 


%For example, during a path lookup, the normal file system will have to walk each component along the path by reading and searching among the directory files which are ultimately backed by disks.
%However, the current file system does not differentiate between data blocks backing a directory file or a regular file.
%Specifically, even though we can know what type this inode is by reading the block containing this inode, there's no guarantee that the REE file system will honestly ask for the data block.
%This can cause problems when a milicious file system directly requests for file data blocks instead of directory file data blocks.
%Therefore, when providing data to the functional component as requested, the secure component should be aware of the block usage and deny any requests for file data blocks.%only grant access to the blocks containing directory files and metadata.
% These directory files are either cached in memory or backed on disks. \note{I shoudn't be talking about cache in here}
%For example, if the malicious file system wants to know the content of a secure file, it can then submit the I/O requests to secure world to obtain the data. 
%However, if the secure world doesn't have any knowledge of the content in the block, it can directly hand in the secure data to the malicious file system.
\end{comment}


\begin{comment}
We base this principle on the insight that 1) file system has the potential to be eidetic as examplified by \cite{eidetic,knockoff}.
and that 2) the cloud can be useful in detecting anomalies as proposed in \cite{jason_determinism}.

This means given a set of inputs, two replica file sytems, on the cloud and the local, if both untampered, will always yield the same outputs, otherwise the outputs will diverge.
\end{comment}

%in a manner similar to remote execution \cite{clonecloud} or operation shipping \cite{coda_shipping}.


%Unless verified, these operations are considered untrusted.
%Eventually, taken the hint from the cloud, the secure component inside TEE can give these operations a greenlight or rejection. %thus ensuring the file system security while still preserving data privacy.
%The cloud doens't replicate the whole image of the disk from the local device. 
%Instead, it only captures the structure of the local file system through replicating metadata.
%Whenever the local device wants to operate on metadata (i.e. create/delete a new file) through the services provided by REE file system, it will also forward the operation to the cloud.
%Then the cloud will perform the same operation to these metadata and report back to the device wether this operation is legit or not.
%Eventually, with the hint from the cloud, we can give the operation a greenlight or reject thus ensuring the file system security while still preserving data privacy.
 

%Much prior work has set sail for complete local secure persistence.
%However, they only solve a part of the puzzle, which usually covers the first three security properties.
%CFS-like systems\cite{cfs} seem to be a promising solution.
%They ensure data integrity, confidentiality and freshness by encrypting data and metadata, and maintaining metadata freshness file as proposed by \cite{plutus,sirius}.
%Open-ended solutions which leverage TEE also set to guarantee secure local persistence.
%OP-TEE\cite{optee} forwards file system API invocations to a handler in normal world.
%Then the handler will ask the file system in normal world to do the rest of the work.
%However, besides having a huge TCB, which allows for a giant attack surface, a common and major vulnerability of these approaches is that they still trust the OS as an honest service provider, a statement which may not hold on IoT devices.
%When in a malicious OS, even though the encrypted cannot be examined, the requests of storing them persistently can be silently dropped, causing the data to lose for good.
%Therefore, It's hard, if not impossible, for prior work to guarantee verifiable persistence.
%And indeed, a large number of optimizations have been done to better the idea\note{cite different works}.
%Unfortunately, they still suffer in two aspects 1) Their TCB is huge which allows for a giant attack surface and they're vulnerable to the compromised OS. 2) The cryptographic operations can drain the device itself. 
%these approaches are vulnerable to DoS attack where the command to write data persistently on disks can be silently dropped.
%When in a malicious OS, even though the encrypted data cannot be examined, the requests of storing them persistently can be silently dropped, causing the data to lose for good.
%The first three have been carefully examined in much prior work.
%But the fourth is hard to guarantee, which will be discussed in the next paragraph.
%2) Small TCB. Unlike prior work that incorporates a full-fledged file system into its TCB, we target a design that has a much more compact TCB enabled by hardware security mechanism. 
%3) Low ovehread. The system should respect the performance constraints and use scenario of IoT devices. All operations should have an affordable overhead. 

%\paragraph{Challenge} Given the above design goals, a critical challenge is how to ensure non-repudiable I/O while having small TCB size as well as afforadable overhead.
%specifically speaking, we not only should guarantee data integrity and confidentiality, but also ensure these data are honestly written to disks.


%\paragraph{Poor connection is common}
\begin{comment}
\paragraph{Prepare for poor connectivity}
IoT devices are often deployed in remote areas~\cite{farmbeats} and connect to the cloud through wireless links. 
Hence, the connectivity is often limited in bandwidth and can be intermittent\cite{iot_gateway}. 
A practical IoT system should efficiently use the network bandwidth, and continue to operate even during network disconnection.
\note{more citations -- check IBM edge computing cited by proposal}
\end{comment}


%When we shed a light on the host of these IoT devices, the cloud, we can find invaluable resources.
%Totally opposite to its tenants, IoT devices, the cloud is more trustworthy in the sense that 1) it allows for more security techniques since it's not bound by performance, 2) it often enjoys professional maintainence and timely patching\cite{googlecloud}.
%However, despite the high availability and reliability the cloud has, it's not the case for the network connection.
%Due to the various environment where the IoT devices can be deployed, one should expect an IoT device to go through much more sufferings in network connection, which can be intermittent and slow.
%In such scenarios, the IoT devices should still be able to operate and store the data persistently and securely. 


\begin{comment}
TrustZone is assumed to boot securely and backs TEE. 
The cloud runs a ``skeleton'' file system for verification. 
The communication between IoT device and the cloud is encrypted and that the messages cannot be forged. 
\end{comment}







%\subsection{Shepherding IoT File System with Cloud}
\begin{comment}
\paragraph{Security is not a one-man job} 
As discussed in \S\ref{sec:motiv}, although prior work has made early attempts to address the above challenges, they fail to address them altogether because relying on normal file system services to carry out I/O operations is their Achilles' heel.
Though there are emerging attempts to defend against the malicious OS and enforce kernel integrity such as hypervisor-based approaches \cite{inktag,haven}, they are usually designed for datacenter and the cloud.
Their price for security is too high in our scenario.
Therefore, we argue that in the unique setting of IoT, \textit{security is not a one-man job}.
\end{comment}

%As discussed in \S\ref{sec:motiv}, although prior work have made early attempts to address the above challenges, they fail to address them altogether. 
%Even with hardware-based mechanism, encryption and key management is still heart to most prior work such as \cite{cfs,sgxlog,plutus,sirius,non-repudiableio}.
%Nevertheless, relying on normal file system services to carry out I/O operations is their Achilles' heel.
%For hypervisor-based approaches\cite{inktag}, which is designed for datacenter and the cloud, their price for security is however too high in our scenario.
%Therefore, we argue that in the unique setting of IoT, \textit{security is not a one-man job}.




\begin{comment}
\paragraph{The best of both worlds}
By far, we have discussed why even with the hardware-based mechanism, file system security, especially verifiable persistence, still can not be ensured solely on the local side and how the cloud can help complete the puzzle.

We propose a framework which sets to exploit the security guarantee provided by the local device and the cloud as whole.
Under this framework, we envision the complete file system security is guarded by the \textbf{cooperation} between the two inseparable parts, which shoulder different security responsibilities.
On the local side, we propose the local device leverages hardware-based mechanism to run the file system at its best efforts, and the cloud, as the indispensable complement, \textbf{shepherds} the file system running on the local device.
Moreover, even with intermittent connection, the local device can securely and persistently store the data.
%Note that the cloud only has to have the metadata and user data doesn't have to be entrusted to the cloud at all.\note{cite data breach in Amazon EC2? will weaken our argument?}
\end{comment}


==> design-goals.tex <==
\subsection{Design Goals and Challenges}

In presence of the powerful adversaries, \sys{} aims to 1) embrace the strong security properties (i.e., data confidentiality, integrity, freshness and verifiable persistence), and 2) facilitate reuse of commodity file systems on IoT devices.
However, with the two goals, we face the following challenges:
\begin{enumerate}
	\item Beyond forging system call to cause data corruption or leakage, a compromised kernel may conduct controlled side-channel to infer the data.
	\item Reusability can only be achieved by delegating file operations.
\end{enumerate}


==> discussion.tex <==
%\begin{comment}
\section{Discussion: Dealing with Cloud Disconnection}

%As has been discussed in \S\ref{sec:rationales}, 
It's not uncommon for IoT devices to experience poor connection with the cloud.
For such a case, 
%We devise mechanisms to keep the \fs{} available even cloud connection is sporadic or down.
we propose two mechanisms for the IoT apps to continue to use \sys{}.
First, the runtime executes the pending, unvalidated data operations. 
For reads, it notifies the app that the return data is untrusted. 
For write, it marks the written pages/blocks as untrusted in case the app wants to read from them later. 
It also checkpoints these pages/blocks in case OFS eventually disagrees on, and rejects the data operations.
Our rationale is to rely on the app's domain method to deal with untrusted data in the face of cloud disconnection.
When the connectivity is recovered, all pending data operations will be validated. 

Second, the runtime allows trusted writes of a limited amount of data even at any time, even when connection is down. 
This is important for system log files. 
To do so, during the file system initialization and the cloud is connected, it creates a fixed-size \textit{emergency} file with pre-allocated blocks.
Since the mapping from file offsets to disk blocks is known, an app can safely execute non-cached write to the file at any moment without validation from the cloud. 
The writes are always trusted. 

%\end{comment}

==> exp-old.tex <==
\section{Early Experience}

\paragraph{Platform}
target platform: omap4, pandaboard. We chose the platform because of XXX. 

Other viable platform: NXP, Beagleboard X15, etc...

\paragraph{Software stack}
Host OS -- Linux 4.4 

Weak core: 
we have already implemented these features... heterogeneous -- for cross ISA execution...

\paragraph{Bootstrapping}

also talk about virtual page setup, carveout memory, etc.

\paragraph{MMU emulation}

\paragraph{DBT engine}
lines of code, etc.

One major challenge is the complexity of DBT engine.

POSIX, strip down existing DBT engine.

Built atop QEMU, We have successfully run a tci backend that essentially interprets the IR. 
The efficiency can be low though, about XXX.
We are building another backend based on ARMv7m (or even ARMv6m). 

We were assuming a clean kernel API (that at least survive across multiple major kernel versions). 
It is hard though, because data structures are passed through the kernel API; and depending on the kernel configuration, the layout (and members) of these data structures can vary differently. 



==> exp_conf.tex <==
% !TeX root = main.tex

%\begin{table}[]
%\centering
%\caption{Kernel support for power sandbox. (X) indicates cost billing mechanism}
%\label{my-label}
%\begin{tabular}{|l|l|l|l|l|l|}
%\hline
%Technique                                                                 & CPU & GPU & DSP & WiFi & MMC \\ \hline
%\begin{tabular}[c]{@{}l@{}}spatial \\ ballooning\end{tabular}       &  Y (usage)  &     &     &      &     \\ \hline
%\begin{tabular}[c]{@{}l@{}}temporal \\ ballooning\end{tabular}          &     &  Y   &  Y   &  Y (net)    &   Y (blk)  \\ \hline
%\begin{tabular}[c]{@{}l@{}}power state\\ virtualization\end{tabular} &  Y   &  Y   &  Y   &  Y    &   Y  \\ \hline
%\end{tabular}
%\end{table}


\begin{table}[t!]
\centering
\caption{Experiment Setup}
\label{exp_setup}
\begin{tabular}{|l|l|l|}
\hline
        & \begin{tabular}[c]{@{}l@{}}Value \end{tabular}  & \begin{tabular}[c]{@{}l@{}}Description 
        \end{tabular} \\ \hline
%iosize     &     8KB                                                                                                                       & Size of a block io request \\ \hline
%count &  1000                                                                                                                          &  Number of write operations\\ \hline
%dsync & false & Indicating synchronous r/w \\ \hline
%world\_switch & 1294 & 
%
%\begin{tabular}{@{}c@{}}  World switch cost \\  in cycles on ARMv8\cite{vtz} \end{tabular}
%
%\\ 
%\hline
%\hline
RTT & 64.5ms & WiFi roundtrip time\\ \hline
Up & 0.94Mbps & WiFi uplink bandwidth\\ \hline
Down & 4.12Mbps & WiFi downlink bandwidth\\ \hline %\hline
%rtt\_lte & 69.5ms & LTE roundtrip time \\ \hline
%up\_lte & 5.64Mbps & LTE uplink bandwidth \\ \hline
%down\_lte & 12.74Mbps & LTE downlink bandwidth\\ \hline

\end{tabular}
\hspace{-20pt}
\end{table}

\begin{comment}
RTT\_lte & 69.5ms & Median LTE RTT
to the cloud\\ \hline
up\_lte & 5.64Mbps & Median uplink throughput of LTE \\ \hline
down\_wifi & 12.74Mbps & Median downlink throuput of LTE\\ \hline
\end{comment}


==> extras.tex <==
\subsection{Inter-processor coordination}

\paragraph{Execution handoff}
%\paragraph{Enter/exit PM core execution}
As mentioned above, the main CPU and the PM core run alternately:
for suspend, the kernel powers off the CPU and moves its execution to the PM core;
at the end of resume, the kernel moves its execution back to the main CPU. 
%We implement the enter/exit as a pair of kernel functions and manually insert the invocations on suspend/resume paths. 
%\paragraph{Execution handoff}

In the execution handoff, we keep the kernel oblivious to the PM core internals. 
Upon moving to the PM core, the kernel passes a snapshot of the CPU state -- containing various register values -- to the \engine{}; 
when the kernel execution leaves the PM core, the \engine{} passes back a snapshot of its \textit{virtual} CPU state. 
This is analogous to virtual-to/from-physical migration in full-fledged virtual machines~\cite{vmware-v2p}; the major difference is that our ``physical'' CPU is much more powerful than the ``host'' -- the PM core.
%Our system differs in that the state of IO devices does not migrate and our ``host platform'' is a very simple core.

%\note{figure: control transfer: normal or exception handling, state involved}

\paragraph{Interrupt routing}
In suspend/resume, the OS relies on interrupts to learn the power states of IO. 
When handoff happens, the responsibility of interrupt handling must be transferred \textit{atomically}, since one interrupt event can only be handled once. 
To do so, the \engine{} populates the PM core's interrupt vectors according to that of the main CPU;
it then redirects future interrupt events from the main CPU to itself (or vice versa), by reconfiguring the platform interrupt controller.
The main CPU, on the other hand, is kept oblivious.


==> fig-block-traces.tex <==
% !TEX root = main.tex
\begin{figure}[h!]
	\vspace{-4mm}
	\centering
	\includegraphics[width=0.4\textwidth{}]{./figs/plot/macrobench/block-traces}
	\vspace{-3mm}
	\caption{Block traces when performing sequential writes to the same file for same size on \code{f2fs} twice, comparing unmodified \code{f2fs} and \code{f2fs} protected by obfuscation surface.
	X-axis: time, Y-axis: block number.}
	\label{fig:block-traces}
	\vspace{-3mm}
\end{figure}


==> fig-eg.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.46\textwidth{}]{figs/rw_seq_large}

	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\vspace{-5pt}		% use as needed
	\caption{Workflows of File I/O. We assume that all read()s and write()s are cached. {OBSOLETE}}
	\label{fig:sequence}
	\vspace{-10pt}		% use as needed
\end{figure}
\begin{comment}
\begin{figure}[!t]
	
	\begin{minipage}[b]{0.23\textwidth}
		\includegraphics[width=1\textwidth]{figs/eg/open}
		        \subcaption{read}
		\label{fig:eval:read}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.23\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/eg/write}
		        \subcaption{write}
		\label{fig:eval:write}
	\end{minipage}	
	~
	\begin{minipage}[b]{0.23\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/eg/read}
		        \subcaption{read}
		\label{fig:eval:fsync}
	\end{minipage}	
	~
		\begin{minipage}[b]{0.23\textwidth}
			%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
			\includegraphics[width=1\textwidth]{figs/eg/fsync}
			\subcaption{fsync}
			\label{fig:eval:fsync}
		\end{minipage}
	%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
	\vspace{-5pt}		% use as needed
	\caption{System Sequence Diagram. We assume after write(), the read() can directly read from secure page cache.}
	\label{fig:sequence}
	\vspace{-10pt}		% use as needed
\end{figure}
\end{comment}

==> fig-macrobenchmarks.tex <==
% !TeX root = main.tex
\begin{figure*}
	\begin{minipage}[b]{0.25\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/macrobench/seq-read}
		        \subcaption{Sequential Read}
		\label{fig:eval:seq-read}
	\end{minipage}
	~
	\begin{minipage}[b]{0.25\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/macrobench/seq-write}
		\subcaption{Sequential Write}
		\label{fig:eval:seq-write}
	\end{minipage}	
	~
	\begin{minipage}[b]{0.25\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/macrobench/rand-read}
		        \subcaption{Random Read}
		\label{fig:eval:rand-read}
	\end{minipage}
	~
	\begin{minipage}[b]{0.25\textwidth}
	%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
	\includegraphics[width=1\textwidth]{figs/plot/macrobench/rand-write}
	\subcaption{Random Write}
	\label{fig:eval:rand-write}
	\end{minipage}	
	\vspace{-15pt}		% use as needed
	\caption{Read/write microbenchmarks with the metadata stencil and operation verifier turned off.
	}

	\label{fig:eval}
\end{figure*}


==> fig-microbenchmarks.tex <==
% !TeX root = main.tex
\begin{figure}[t!]
	\begin{minipage}[b]{0.15\textwidth}
		\includegraphics[height=1\textwidth]{figs/plot/ubench/msg-passing}
		        \subcaption{Message Passing}
		\label{fig:eval:msg-passing}
	\end{minipage}
	\begin{minipage}[b]{0.15\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[height=1\textwidth]{figs/plot/ubench/metadata-stencil}
		        \subcaption{Metadata Stencil}
		\label{fig:eval:metadata-stencil}
	\end{minipage}	
	\begin{minipage}[b]{0.15\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[height=1\textwidth]{figs/plot/ubench/op-verifier}
		        \subcaption{Operation Verifier}
		\label{fig:eval:op-verifier}
	\end{minipage}	
	%\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
	\vspace{-5pt}		% use as needed
	\caption{A list of microbenchmarks
	}

	\label{fig:eval}
\end{figure}


==> fig-path-traversal.tex <==
\begin{figure}
	\centering
	%\missingfigure[figwidth=0.45\textwidth]{Components and channels to be protected by overwatch, including all discussed later}
	\includegraphics[width=0.46\textwidth{}]{./figs/plot/macrobench/path-traversal}
	\label{fig:path-traversal}
	\caption{Path traversal latency}
\end{figure}


==> fig-real.tex <==
% !TeX root = main.tex
\begin{figure}%{R}{0.25\textwidth}
	%\vspace{-2mm}
	\centering
	%\missingfigure[figwidth=0.45\textwidth]{Components and channels to be protected by overwatch, including all discussed later}
	\includegraphics[width=0.25\textwidth{}]{./figs/plot/macrobench/filebench/real}
	\caption{Throughput comparison of intelligent camera apps under different network latencies.}
	\label{fig:real}
	%\vspace{-2mm}
\end{figure}


==> fig_latency.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
	\begin{minipage}[b]{0.15\textwidth}
		\includegraphics[height=1.1\textwidth]{figs/plot/read}
		        \subcaption{read}
		\label{fig:eval:read}
	\end{minipage}
	\begin{minipage}[b]{0.15\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[height=1.1\textwidth]{figs/plot/write}
		        \subcaption{write}
		\label{fig:eval:write}
	\end{minipage}	
	\begin{minipage}[b]{0.15\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[height=1.1\textwidth]{figs/plot/fsync_2}
		        \subcaption{fsync}
		\label{fig:eval:fsync}
	\end{minipage}	

	%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
	\caption{A comparison of file I/O latencies
%	\psbox{} ensures fairness by keeping throughputs of other apps largely unchanged.
	}
	\vspace{-15pt}		% use as needed
	\label{fig:eval}
\end{figure}


==> introduction-liwei.tex <==
% !TEX root = main.tex

\section{Introduction}
\label{sec:intro}

%\note{The intro words about IoT can be cut. Likely you'll need one sentence for that. You then should quickly move to talking about the file systems for IoT/edge. Then you will say what's wrong with existing designs and present your threat model.}

%\note{The flow: talking about the transition from mobile to IoT -- People are becomming more connected, IoT edge processing is becoming popular (I hate the phrase, must rephrase), IoT devices are XXX, example use are XXX, they play an invaluable role in future world}

%Thanks to the emerging Internet-of-Things(IoT) devices, we've never become so connected. % we->people? less subjective

% Mobile devices connect people to each other.
% IoT devices weave a web of inter-connected nodes..XXX 

%\note{IoT needs secure storage.}

Emerging IoT devices are promise to future edge processing. 
A prominent use of these devices is smart sensors. 
Smart meters measure power consumption thus enabling smart grid\note{cite}; smart temperature and humidity sensors digitalize the environment and can thus help make a better living condition\note{cite}. 
These device have a nature to store data.
In the case of sensors, they'll need to store the capturd data for post analysis; in other scenarios, they'll need to store system configurations, credentials, user information, etc.
However, due to the tight budget, they are usually wimpy and vulnerable.
As a result, attacks against other platforms can easily be launched against these devices which usually carry sensitive data.
To worsen the situation, the connection between the device and the cloud can be intermittent and unstable.
This makes entrusting the data solely to the cloud an unreliable solution.

Therefore, IoT devices demand secure local storage.
And we identify the security requirement as four properties such storage system must gurantee 1) \textbf{freshness}: the system must provide the latest version of data. This elimites swapping attack. 2) \textbf{data integrity}: the data must not be rigged during execution. This eliminates XXX attack. 3) \textbf{data confidentiality}: the data content must not be exposed to any third party. This eliminiates XXX attack. 4) \textbf{non-repudiable I/O}: the data must be stored honestly to its destination. This eliminiates XXX attack.

\note{this paragraph is too fat}
Current approaches targeting different platforms mainly take two routes to the four properties. 
The first approach is targeting local device based on the idea of execution isolation.
The isolated exeuction environment is called Trusted Execution Environment (TEE), which gurantees the integrity and confidentiality of code and data inside.
Open Portable Trusted Execution Environment (OP-TEE) leverages ARM TrustZone to implement TEE.
However, it forwards operations to a handler in normal world to carry out operations.
%Put these into related work
%Inktag, Trustvisor, Overshadow use specialized hypervisor to isolate execution evironment and monitor memory changes in host machine. VirtualGhost adds compiler instrumentation to OS code to create isolated memory region. 
The second approach is targeting the cloud server based on cryptographic file system (CFS) \note{cite}.
Plutus, SiRiUS and other homogeneous work guanrantee data confidentiality and integrity by encrypting data and metadata.
%Ideal as they may sound, 
However, these approaches are not easily applicable in the IoT era.
Major drawbacks include the execeedingly large Trusted Computing Base(TCB) and performance overhead. 
OP-TEE relies on the file system in normal world whose code base is huge, complex and buggy\note{cite remzi FAST13}; 
CFS-like systems suffer from excessive operations on encryption and decryption, which cannot be efficiently handled by IoT devices.
To make things worse, IoT devices have a more critical threat model which invalidates much of the prior TCB such as trusted OS or trusted storage.
Like its counterpart--the cloud, they're designed to be always connected to the Internet;
however, unfortunately, unlike its counterpart, they often receive the poorest software support.
This brings new challenges to IoT security.
On one hand, the threat is not new.
There can be a powerful party of interest which has \textbf{full} control of the device's software stack.
%On the other hand, these IoT devices don't usually enjoy timely patch and maintainance as the cloud and they suffer from performance.
On the other hand, these devices need to securely store their data locally in the sense that the four security requirements must be met.
%Therefore we envision a powerful party of interest which can have \textbf{full} control of the device's software stack.

%Our approach
%Having noticed hardware-assisted protection such as Intel SGX and ARM TrustZone can provide strong isolation gurantee, 
% we propose that securing IoT fs is not a one-man job
 
To this end, we propose to reconstruct the IoT file system by combining the best of both worlds. 
We base our design on the insight that, on the local device, the hardware mechanism provides the strongest isolation guanrantee; on the cloud, the software stack enjoys the most timely patch and professional management. 
%Specifically, we leverage TrustZone to secure data and the cloud to secure metadata.
%To describe our design in a nutshell, we secure the data locally leveraging TEE and the structure of the data (i.e. the metadata) remotely on the cloud.


To describe our design in a nutshell, we propose the secure IoT file system 1) host \textit{secure cache} inside TEE, 2) manage its \textit{replicated metadata} on the cloud and 3) be aware of its \textit{block usage}.
%We reflect any untrusted changes to the local metadata on the cloud and the cloud will validate untrusted local reads/writes.
The architecture is shown in Figure~\ref{fig:overview}.
%separting security-critical data into secure world by leveraging ARM TrustZone which is hardware-assisted and provides strong security gurantee. 

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.47\textwidth{}]{./figs/arch2} 
	%\missingfigure[figwidth=6cm]{Juno platform power instrumentation}
	\caption{An overview of this work}
	\label{fig:overview}
	\vspace{-10pt}		% use as needed
\end{figure}

%In the secure world, we handle only . 
%In the normal world, we run a commodity file system to execute complex logic. 
%From the application's perspective, they're oblivious of the secure world and interact normally with the underlying file system via system calls as usual. 
%When the read/write is cached in memory, operations stay in the secure world.
%Otherwise, operations still have to go through the actual file system in the normal world.
%However, this is not enough to guard against a malicious file system which can conduct rollback attack\note{cite} since it can corrupt any commands issued by the user at will.
%To guard against rollback attack \note{cite} which is easily done by a malicious file system, we re-route the call to the underlying block layer back to secure plane.
%To ensure non-repudiable I/O, we re-route the call to the underlying block layer back to secure world.
%We buffer all the writes in sequence and verify the unique identifiers (i.e. inode and block number) in them with the cloud, which is trusted and runs a mirror process as a reference.

Our contributions in this work are twofold:
\begin{itemize}
	\item We propose a novel file system design.\note{idea is secure data is stored locally, secure metadata is stored remotely. By storing data using TrustZone, we guanrantee data security; by using the cloud, we gurantee the file system skeleton security.}
	\item We evaluate our design on Linux file system using filebench and iozone benchmarks. The results show our design only incurs \note{XXX} performance overhead and is promising. 
\end{itemize}



==> macro-apps.tex <==
% !TEX root = main.tex

Real-world applications



==> methodology-old.tex <==
% !TEX root = main.tex

\section{Design Sketch}

Given that suspend/resume procedure is time-consuming and IO bound, our key insight is that its efficiency can benefit from extremely asymmetric CPU cores. 
\paragraph{Architectural assumption}
Power domain, wakeup source, shared memory, different ISA, ....
Conceptually, such a weak core is capable of performing suspend/resume on behalf of the strong cores.
In particular, we seek to minimizing the on time of strong cores by offloading the execution of suspend/resume to a weak core. 
%The key idea is to move IO power management to the small cores. 
%enable the kernel to offload the time-consuming IO power management to small cores. 

This seemingly simple goal raises a great deal of challenges, in particular from kernel complexity. 
First, as discussed in Section XXX, the OS code for suspend/resume is complex and invokes a variety of other kernel subsystems.
Second, the hardware discrepancy -- from ISA to memory model -- between asymmetric cores can be huge. 
Third, 

\paragraph{Reflection on K2}
In our prior work K2~\cite{k2} we explored the design of spanning one OS image over highly asymmetric processors. 
As a generic approach for OS refactoring, OS argues for ....
One major drawback of this approach, as we found out in practice, is that it tightly couples the kernel instances (software stack instances) running on different processors. 
This entails two requirements: 
first, the kernel images (as their respective native binaries) must be generated from one unified kernel tree, and every memory object must be placed at the same virtual address;
second, the weak core must run a full-fledged Linux (VM enabled). 
The resultant efforts are substantial (and repetitive) across Linux kernels of different versions or for different SoCs: 
it requires porting kernel trees (e.g. for x86 or ARMv7) to the weak core (which, due to its embedded profile, often receives poor or no support from the mainline kernel) and manual tweaking of kernel configurations, linker commands, and the internal memory layout of data structures.

However, treating a specific, IO-bound kernel procedure (suspend/resume) allows us to explore a design point that is other than K2: 
we trade the kernel execution overhead of the weak core for minimizing coupling and efforts craft the kernel \textit{per se.}.
Thus, we take an extreme design point -- using the weak core as a (software-accelerated) virtualization engine for host kernel execution -- only the suspend/resume path.
This new perspective enables us to retrofit rich results in virtualization.

The top challenge, however, is execution efficiency: 
the weak core has to execute binary in a different ISA;
this, combined with its lack of hardware features (e.g. no MMU or virtualization hardware), may lead to 

\Paragraph{Programming challenge}

This has to be done in software. registers have to be saved and restored. drivers have to decide the PM policies and the order of suspending.

the little PM core -- for efficiency, can be very wimpy. We simply do not assume it has virtual memory hardware. It, however, has access to the DRAM.

(can it access the main DDR? shall we design under memory constraints? this may enable sensor hubs with limited local memory, making our work more generic)


Heterogeneity -- the PM core and the main CPU may differ on ISAs (even ARM cores start to move to 64 bits)
Simply cannot ask for homogeneity.

\Paragraph{Interrupt handling}



==> new.tex <==
% !TEX root = main.tex
\paragraph{A Minimal Example}
\note{the following may be useful. but need revision and compression}
To illustrate our initial design, we next describe a file API sequence, in which a client first open()s a file, read()s and write()s to it, and invokes fsync() to make the changes persistent. 

The interaction sequence of our system is shown in Figure \ref{fig:sequence}.
These syscalls invoke file system functions to read required block and saturate memory pages with the data.
First, open() is issued by a secure application out to the file system in normal world. 
% allocates an entry in the file table owned by the process. 
Open() gathers the metadata (i.e., inode) of the file and sets up a descriptor for the file to be operated on by iteratively querying the super blocks.
Then, the normal file system walks each (sub)directory along the file path by reading metadata and directory file blocks from TEE to do name comparison 
until it finally reaches the metadata block representing the file we want to open and reads it into memory.
As has been described, our system will pass all the queried super blocks directly out to the file system in normal world as they are metadata.
After getting the in-memory inode of the opened file, the physical location of the file on disks is also known and the file's address space is associated with its entry (i.e. file descriptor) in the file table.
When the secure app wants to read() the opened file, our system will first search among the secure page cache.
A cache hit will return the file data directly to the app.
In case of a cache miss, our system issues read() out to the normal world and sends the same request to the cloud simultaneously.
Then it will examine all incoming block read requests from normal world and validate them with the cloud.
If the validation succeeds (i.e., matching that with the cloud), those blocks are read to fill page cache and returned to the secure app.
Otherwise, the read() will fail. 
%This is for mmap()
mmap() associates the address space of the process with the inode.
It will locate (if necessary, allocate) page cache for this file then setup the entries of the process's page table to corresponding pages.
User can then read/write the file the same way as they do to a memory region.
Similar to read(), when the secure app write() data to the file, our system will first search among secure page cache. 
A cache hit will make our system write data only to the corresponding page cache. 
Otherwise, our system will forward the write() to normal world so that it can allocate blocks for the write().
Subsequently, our system examines and validates all the incoming block write requests with the cloud.

%each block request is forwarded to the cloud for verification and the new page mapping will also be forwarded for bookkeeping purpose.
%Then the content to be written is copied from user space to these pages.
%Unless an explicit sync is requested, these pages will only be marked dirty without being flushed to disk.
%until an fsync() is called or the system decides to flush all dirty pages.
When changes need to become persistent, the secure app invokes fsync() to flush all dirty pages into the storage.
It scans through all dirty pages of the file and issues block write request accordingly.
These block write requests will be forwarded altogether to the cloud for validation.
%as fsync() acts like a contract between normal world and TEE.
A successful return on fsync() indicates that up to this point, each read/write is validated to be trusted.
%In the case of direct I/O, read() and write() will bypass page cache and directly interact with the block layer.
%Following our design principle, we intercept page cache and block operations.
%As illustrated in Fig \ref{fig:sequence}, TEE hosts all page cache of the secure application. 
%Each request asking for these pages will be directed to TEE then TEE will directly turn in these pages to the secure application.
%Moreover, each block request will be examined by secure world for the security state and usage type as described in \S\ref{sec:block_aware}.


==> obliviousness.tex <==
% !TeX root = main.tex
\subsubsection{Oblivious block traces}

\input{fig-block-traces}

\note{this can go}

We experimentally demonstrate how obfuscation surface keeps \sys{} execution oblivious to an untrusted \fs{}. \note{always summarize result first}

In the experiment, a secure app opens a file and sequentially writes 256KB to it, where all each file operation are delegated to native \code{f2fs}, and \code{f2fs} protected by obfuscation surface with obfuscation level 5 and level 10, with respect to~Figure \ref{fig:block-traces} (a)-(c).
In each scenario, we run the experiment twice, reboot between runs to eliminate cache effects, and collect the block traces requested by the untrusted \fs{}.
As can be seen in Figure~\ref{fig:block-traces} (a), without obfuscation surface, the file operation delegated in two runs yield exactly same block traces observed by the untrusted \fs{}, which leads to access pattern exposure.
However, as demonstrated in~Figure \ref{fig:block-traces} (b) and (c), after the obfuscation surface, same delegated file operations yield two largely different block traces observed by an untrusted \fs{}.
As a result, an untrusted \fs{} cannot infer the access pattern of \sys{} or the directory structure of the file, because it is blinded as to which file operation is intended by \sys{}.
%We conduct an experiment to show the block traces when accessing the same file at the offset, as observed by normal world with and without obfuscation surface.
%\todo[inline]{TBD}
%show that system cannot differentiate between different file reads.
%\note{an attack -- defense mechanism table}

%\note{a figure that has components and vulnerabilities illustrated}


==> opt.tex <==
% !TEX root = main.tex

\section{Discussions}

Though without any optimizations, the overhead of waiting for the cloud verification is unaffordable, several optimizations are easily foreseeable.

\paragraph{Cached outcomes} 
A straightforward technique to reduce latency is to use cache.
Since each I/O request is a tuple containing $<blk\_no, page\_addr, len, offset>$,
each time such a message is sent to the cloud, a response can be cached in TEE and used later.

\paragraph{Evaluate block trustworthiness}
Current checkpoints will blindly checkpoint each write.
App can only access trusted block
Writes will update block status and invalidate trustworthiness until verified
Checkpoint existing content 

%\paragraph{Batched verification}
%A major overhead is introduced by the network latency.







==> tab-rpc.tex <==
% !TeX root = main.tex
\begin{table}[h]
%\begin{minipage}[]{0.6\textwidth}
	\fontsize{8.0}{9.0}\selectfont
	\begin{center}
%		\begin{tabular}{@{}l|@{}c|@{}l|
%				@{}l@{}l@{}l@{}l@{}l|
%				@{}l|@{}c|@{}l|@{}l}
		\setlength\tabcolsep{3pt}	% hp table insidem margin
		\begin{tabular}{
%				@{}l@{$\;\;$}p{1mm}	% System
				l   
				l	% Attack
				l	% Attack Vector
				l	% Impacts
			}
			% <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
			\hlineB{2.5}
			\textbf{ } &
			\textbf{100} &
			\textbf{100K} & 
			\textbf{1 Million}  
%			\cellcolor{lightgray}\textbf{Operator in TEE.} &			
%			\cellcolor{lightgray}\textbf{MT} &
%			\cellcolor{lightgray}\textbf{Memory} &
%			\cellcolor{lightgray}\textbf{Attestation}
			\\ 
%			$\alpha$ & $\beta$ & $\gamma$ \\
			\hlineB{1.5}
RPC cost				 	
& 100
& 10000
& 1000000\\

\hlineB{2.5}
%Glamdring~\cite{glamdring}	 	 & stream			& SGX	& n/a\\
		\end{tabular}
		\vspace{2mm}
		\caption{Time taken of RPC ping-pong, upon each SVC, TEE directly returns.}
		\vspace{-2mm}
		\label{tab:rpc}
	\end{center}
%\end{minipage}
\end{table}
